Improving Diffusion Models for Authentic Virtual Try-on in the Wild

This paper considers image-based virtual try-on, which renders an image of a person wearing a curated garment, given a pair of images depicting the person and the garment, respectively. Previous works adapt existing exemplar-based inpainting diffusion models for virtual try-on to improve the naturalness of the generated visuals compared to other methods (e.g., GAN-based), but they fail to preserve the identity of the garments. To overcome this limitation, we propose a novel diffusion model that improves garment fidelity and generates authentic virtual try-on images. Our method, coined IDM-VTON, uses two different modules to encode the semantics of garment image; given the base UNet of the diffusion model, 1) the high-level semantics extracted from a visual encoder are fused to the cross-attention layer, and then 2) the low-level features extracted from parallel UNet are fused to the self-attention layer. In addition, we provide detailed textual prompts for both garment and person images to enhance the authenticity of the generated visuals. Finally, we present a customization method using a pair of person-garment images, which significantly improves fidelity and authenticity. Our experimental results show that our method outperforms previous approaches (both diffusion-based and GAN-based) in preserving garment details and generating authentic virtual try-on images, both qualitatively and quantitatively. Furthermore, the proposed customization method demonstrates its effectiveness in a real-world scenario. More visualizations are available in our project page: https://idm-vton.github.io

==> figures/main/ablation_customization.tex <==
\begin{figure}[t]
    \small\centering
    \includegraphics[width=1.0\textwidth]{resources/main/ablation_customization.pdf}
    \vspace{-5pt}
    \caption{
    \textbf{Effect of customization.}
    We compare the generated virtual try-on images of default {\sname} (left) and customized {\sname} (middle and right). We perform customization under two different settings, providing an image of person only (middle) and images of person-garment pair (right). The reference images used in customization are shown in the corner of each image. After customization, \sname~better preserves the identity of garment (\emph{e.g.}, text rendering and patterns) and images are more natural. Also, providing images of person-garment pair generates more authentic images compared to solely utilizing an image of person.
    }
    \label{fig:adaptcompare}
    \vspace{-10pt}
\end{figure}


==> figures/main/adaptation.tex <==

% \begin{figure}[t]
%     \small\centering
%     \includegraphics[width=0.99\textwidth]{resources/main/method2.pdf}
%     \vspace{-5pt}
%     \caption{
%     \textbf{Generated images of virtual try-on using CustomVTON}. 
%     (a) Comprehensive captioning for garment. To fully exploit the text-to-image prior of diffusion model, we extract detailed captions from garment using captioner fine-tuned on fashion dataset. 
%     (b) Our diffusion-based virtual try-on method, coined \emph{CustomVTON}, is able to generate person image with high degree of consistency to the garment image, with better naturalness.
%     Furthermore, we propose \emph{CustomVTON}$^+$, which adapts the model with few reference images of person wearing same garment, further enhances the fidelity to the garment image and image quality (\emph{e.g.}, the text rendering under the pattern, and naturalness within the sleeves). Best viewed in color, zoomed in on monitor. 
%     % by adapting the model with few reference images of person wearing garment,  adapting the model CustomVTON
%     % high fidelity to the garment
%     % in an image of person wearing a garment,  given by an garment image, it struggles to preserve the identity (\emph{e.g.}, pattern in the sweatshirts). 
%     % Our proposed method, \emph{CustomVTON}, is able to generate a
%     % Given an image of human in real world setting and an image of garment, previous Virtual try-on methods struggle to generate a natural try-on image while preserving the details of the garment. However, our method successfully generates highly realistic try-on images that capture the fine-details of the garment. Furthermore, we improve the try-on performance even further through the proposed adaptation method using reference human images wearing the same garment.
%     }
%     \label{fig:teaser}
% \end{figure}
% % \vspace{-30pt}




==> figures/main/qualdress.tex <==
% \begin{figure}[t]
%     \small\centering
%     \includegraphics[width=0.98\textwidth]{resources/main/qual_dress.pdf}
%     % \vspace{-5pt}
%     \caption{
%     \textbf{Qualitative comparisons on dresscode dataset} }
%     \label{fig:qual_dress}
%     % \vspace{-5pt}
% \end{figure}





==> figures/main/teaser_new.tex <==

\vspace{-10pt}
\begin{figure}[ht]
    \small\centering
    \includegraphics[width=0.99\textwidth]{resources/main/teaser_new.pdf}
    \vspace{-10pt}
    \caption{..}
    % \textbf{Generated images of virtual try-on using CustomVTON}. 
    % Prior diffusion-based virtual try-on model~\cite{kim2023stableviton} (\emph{i.e.}, baseline) struggles to capture the details of a garment (\emph{e.g.}, the pattern in the sweatshirts) and generated image lacks naturalness.
    % Our diffusion-based virtual try-on method, coined \emph{CustomVTON}, is able to generate person image with high degree of consistency to the garment image, with better naturalness.
    % Furthermore, we propose \emph{CustomVTON}$^+$, which adapts the model with few reference images of person wearing same garment, further enhances the fidelity to the garment image and image quality (\emph{e.g.}, the text rendering under the pattern, and naturalness within the sleeves). Best viewed in color, zoomed in on monitor. }
    
    % by adapting the model with few reference images of person wearing garment,  adapting the model CustomVTON
    % high fidelity to the garment
    % in an image of person wearing a garment,  given by an garment image, it struggles to preserve the identity (\emph{e.g.}, pattern in the sweatshirts). 
    % Our proposed method, \emph{CustomVTON}, is able to generate a
    % Given an image of human in real world setting and an image of garment, previous Virtual try-on methods struggle to generate a natural try-on image while preserving the details of the garment. However, our method successfully generates highly realistic try-on images that capture the fine-details of the garment. Furthermore, we improve the try-on performance even further through the proposed adaptation method using reference human images wearing the same garment.}
    \label{fig:teaser}
\end{figure}
\vspace{-20pt}


==> figures/table_adapt.tex <==
\begin{table}[t]
    \centering\small
    \caption{\textbf{Quantitative results on in-the-wild, one-shot adaptation} paired images }
        % \resizebox{0.8\textwidth}{!}{
        \begin{tabular}{lccc}
        \toprule
        Method & LPIPS  ($\downarrow$) & SSIM  ($\uparrow$)\\
        % & User  ($\uparrow$) \\
        \midrule

        \sname (ZeroShot) & 0.1642 &0.795 &\\
        \sname (LoRa(r=256))& 0.1573 & 0.794 & \\
        \sname (U-Net)&0.1512 & \textbf{0.797} & \\
        \midrule
        \textbf{\sname (decoder)}& \textbf{0.1502} & \textbf{0.797} & \\

        \bottomrule
        \label{tab:adapt}
        \end{tabular}
% }
        % \caption{Table 1 for VitonHD test dataset}
        
\end{table}



==> figures/table_dresscode.tex <==
\begin{table}[t]
    \centering\small
    \caption{\textbf{Quantitative results on cross dataset (VITON-HD to DressCode).} 
    We evaluate the models trained on VITON-HD dataset on a subset of DressCode dataset for upper body garments. 
    \textbf{Bold} and \underline{underline} denote the best and second best result, respectively. (R) indicates the utilization of RePaint~\cite{lugmayr2022repaint}.}
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{llcccc}
    \toprule
    Base model & Method & LPIPS ($\downarrow$) & SSIM ($\uparrow$) & FID ($\downarrow$) 
    & CLIP-I ($\uparrow$)\\
    % & User  ($\uparrow$) \\
    \midrule
    \multirow{2}{*}{GAN} & HR-VITON~\cite{lee2022high} &0.112 & 0.910& 21.42 & 0.771\\
    & GP-VTON~\cite{xie2023gp} &0.484 &0.780 & &0.628\\
    \midrule
    \multirow{3}{*}{DMs} & DCI-VTON~\cite{gou2023taming} &0.162 &0.893 & 17.63 &0.777 \\
    & LaDi-VTON~\cite{morelli2023ladi} & 0.149 & 0.905 & 16.54 & 0.803\\
    & Stable-VITON~\cite{kim2023stableviton} & 0.152 & 0.895 & 14.37 & 0.819\\
    \midrule
    % \textbf{Ours(CLIP-Encoder)}&0.121   &0.850  & 7.26 \\
    DMs & \textbf{\sname}&\textbf{0.062}   &\textbf{0.920}  &\textbf{8.64} &\textbf{0.904} \\
    % \textbf{Ours(UNet-Encoder, RePaint)}&\textbf{0.099}   &0.884  & 6.20 \\
    % \sname \textbf{Ours}&\textbf{0.099}   &0.884  & 6.20 \\
    \bottomrule
    \end{tabular}
     }

    % \caption{Table 1 for VitonHD test dataset}
    \label{tab:main1}

\end{table}



==> figures/table_humanonly.tex <==
\begin{table}[t]
    \centering\small
    \caption{\textbf{Quantitative results on in-the-wild, one-shot adaptation, human image only} }
        \resizebox{0.96\textwidth}{!}{
        \begin{tabular}{lccc}
        \toprule
        Method & LPIPS  ($\downarrow$) & SSIM  ($\uparrow$) &  CLIP-I ($\uparrow$) \\
        % & User  ($\uparrow$) \\
        \midrule
        \sname (0-Shot) & 0.1691 &0.784 &0.8862 \\
        \sname (LoRA(r=256))&0.1653  & 0.7866 & 0.8945 \\
        \sname (U-Net)&0.1584 &0.7908  &0.9032 \\
        \midrule
        \textbf{\sname (decoder)}& \textbf{0.1561} &\textbf{ 0.792} &\textbf{0.9088} \\

	
        \bottomrule
        \end{tabular}
}
        % \caption{Table 1 for VitonHD test dataset}
        \label{tab:main1}
\end{table}

	
